Asymptotic Behaviors and Phase Transitions in Projected Stochastic Approximation: A Jump Diffusion Approach

In this paper we consider linearly constrained optimization problems and propose a loopless projection stochastic approximation (LPSA) algorithm. It performs the projection with probability $p_n$ at the $n$-th iteration to ensure feasibility. Considering a specific family of the probability $p_n$ and step size $\eta_n$, we analyze our algorithm from an asymptotic and continuous perspective. Using a novel jump diffusion approximation, we show that the trajectories connecting those properly rescaled last iterates weakly converge to the solution of specific stochastic differential equations (SDEs). By analyzing SDEs, we identify the asymptotic behaviors of LPSA for different choices of $(p_n, \eta_n)$. We find that the algorithm presents an intriguing asymptotic bias-variance trade-off and yields phase transition phenomenons, according to the relative magnitude of $p_n$ w.r.t. $\eta_n$. This finding provides insights on selecting appropriate ${(p_n, \eta_n)}_{n \geq 1}$ to minimize the projection cost. Additionally, we propose the Debiased LPSA (DLPSA) as a practical application of our jump diffusion approximation result. DLPSA is shown to effectively reduce projection complexity compared to vanilla LPSA.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> append/append_distributed.tex <==
\section{Special Condition: Distributed Learning}\label{sec:sp_fedavg}
In this section, we focus on the specific case of distributed learning. 
Recall that we have introduced the distributed optimization problem \eqref{eq:dis_opt} in Section~\ref{sec:example}. 
We first 
% present the FL problem and 
establish the equivalence between LPSA and local SGD 
% Then we 
and then
restate our main results under the context of distributed learning.
We also discuss related works on distributed optimization.

\subsection{The Problem and Reduction}
In this subsection, we 
% formulate our algorithm in federated settings and 
show that LPSA is equivalent to local SGD.
% Before we proceed, we first give the formal statement of our algorithm
% \begin{algorithm}[h]
% \caption{Loopless Projected Stochastic Approximation (LPSA)}
%  	\label{alg:lp_proj_sa}
%  	\begin{algorithmic}
%  		\STATE {\bfseries Input:} function $f$, data distribution $\gD$, initial point $\vx_0$, step size $\eta_n$, projection probability $p_n$.
%  		\STATE {\bfseries Initialization:} let $\bfx_{0}^{(k)} = \bfx_0$ for all $k$.
%  		\FOR{$n=0$ {\bfseries to} $T-1$}
%  		 \STATE{Sample $\zeta_n\sim \gD$ and $\omega_n\sim \mathrm{Bernoulli}(p_n)$}
%  		 \STATE{$\vx_{n+\frac{1}{2}}=\vx_n-\eta_n\nabla f(\vx_n,\zeta_n)$}
%  		 \IF{$\omega_n=1$}
%  		  \STATE{$\vx_{n+1}=\gP_{\mA^\bot}\vx_{n+\frac{1}{2}}$}
%  		 \ELSE
%  		  \STATE{$\vx_{n+1}=\vx_{n+\frac{1}{2}}$}
%  		 \ENDIF
%  		 \ENDFOR
%  		\STATE {\bfseries Return: $\gP_{\mA^\bot}\vx_T$.}
%  	\end{algorithmic}
% \end{algorithm}

% For typical distributed optimization problems, we can rewrite them as a global consensus problem,
% \begin{equation}\label{eq:dis_opt}
%  \min\limits_{\vx^{(1)},\vx^{(2)},\dots,\vx^{(N)}}\frac{1}{N}\ssum{k}{1}{N}\sE_{\zeta^{(k)}\sim\gD_k} g(\vx^{(k)},\zeta^{(k)}) ~~\text{ s.t. } \vx^{(1)}=\dots=\vx^{(N)},
% \end{equation}
% where there are $N$ clients, $\vx^{(k)}$ is the local parameter at the $k$-th client and $\zeta^{(k)}$ represents the randomness from this client.
% If we concatenate all the local parameters as $\vx=\left[(\vx^{(1)})^\top,(\vx^{(2)})^\top,\dots,(\vx^{(N)})^\top\right]^\top\in\sR^{Nd}$ and 
% $\zeta = ( \zeta^{(1)}, \zeta^{(2)}, \dots, \zeta^{(N)} )^\top$,
% % $\zeta = (i, \zeta^{(i)})$
% we can rewrite the equation \eqref{eq:dis_opt} as the form of equation \eqref{eq:proj_opt}, where
% % $f(\vx, \zeta) = \sum_{k=1}^n \mathbbm{1}$
% $f(\vx, \zeta) = \frac{1}{N} \sum_{k=1}^N g( \vx^{(k)}, \zeta^{(k)} )$,
% $\gD = \gD_1 \times \gD_2 \times \cdots \times \gD_N$
% % $\gD=\frac{1}{n}\ssum{k}{1}{n}\gD_k$
% and $\vA^\top$ is equipped with a particular structure
% \begin{equation}\label{eq:mat_A_fl}
%     \vA^{\top}=\begin{bmatrix}
%     \rmI_d & -\rmI_d & \vzero_d & \cdots & \vzero_d & \vzero_d\\
%     \vzero_d & \rmI_d & -\rmI_d & \cdots & \vzero_d & \vzero_d\\
%     \vdots & \vdots & \vdots & \ddots & \vdots & \vdots\\
%     \vzero_d & \vzero_d & \vzero_d & \cdots & \rmI_d & -\rmI_d
%     \end{bmatrix}\in \sR^{(N-1)d\times Nd}.
% \end{equation}
% In the expression of $\mA^\top$, $\rmI_d \in \sR^{d \times d}$ is the identity matrix and $\vzero_d \in \sR^{d \times d}$ is the zero matrix.
% For such an $\mA$, 
With $\mA$ defined in \eqref{eq:mat_A_fl},
the operators $\gP_{\mA^\bot}$ and $\gP_{\mA}$ are easy to compute.
One can check that
\begin{align}\label{eq:proj_A_bot_fl}
\gP_{\mA^\bot} (\vx) = \left[ \bar{\vx}^\top, \bar{\vx}^\top, \cdots, \bar{\vx}^\top \right]^\top  
\end{align}
and
\begin{align*}
% \label{eq:proj_A_fl}
\gP_{\mA} (\vx) = \left[  (\vx^{(1)} - \bar{\vx})^\top,  (\vx^{(2)} - \bar{\vx})^\top, \cdots,  (\vx^{(N)} - \bar{\vx})^\top \right]^\top,
\end{align*}
where $\bar{\vx} = \frac{1}{N} \sum_{i=1}^N \vx^{(i)}$.
Then we can establish the equivalent between LPSA and local SGD.
At iteration $n$, the step $\vx_{n + \frac{1}{2}} = \vx_{n} - \eta_n \nabla f (\vx_n, \zeta_n)$ represents a step of local update, that is
$\vx_{n + \frac{1}{2}}^{(k)} = \vx_n^{(k)} - \eta_n \nabla g ( \vx_{n}^{(k)}, \zeta_{n}^{(k)} ) $ for each $k$.
If $\omega_n=1$, 
the projection step $\vx_{n+1} = \gP_{\mA^\bot} (\vx_{n + \frac{1}{2}} ) $ becomes
 a round of communication such that all the local parameters share the same value, i.e., $\vx_{n+1}^{(k)} = \frac{1}{N} \sum_{i=1}^N \vx_{n + \frac{1}{2} }^{(i)}$ for each $k$; if $\omega = 0$, no communication happens and $\vx_{n+1}^{(k)} = \vx_{n + \frac{1}{2} }^{(k)}$.
 Finally, Algorithm \ref{alg:lp_proj_sa} returns the average of all local parameters $\gP_{\mA^\bot} \vx_T = \frac{1}{N} \sum_{k=1}^N \vx_{T}^{(k)}$.
 
 
 The above reduction analysis implies that under the context of distributed learning, Algorithm \ref{alg:lp_proj_sa} becomes a loopless version of local SGD.
 The main difference between LPSA and original Local SGD is that LPSA has a stochastic length of local updates, which is determined by how frequently we observe $\omega_n = 1$.
 Since $p_n$ gradually decreases, the expectation of local updates would gradually increase.
 Such a difference does not deteriorate the convergence under certain conditions, as shown in Theorem \ref{thm:converge}.
Moreover, the probabilistic loop also facilitates theoretical analysis.

\subsection{Restatement of Theoretical Results}
In this subsection, we examine the theoretical results and give a revision of Theorem \ref{thm:counter} under the FL condition.

For simplicity, we define the population loss function on client $k$ as $g_k (\vx^{(k)}) := \sE_{ \zeta^{(k)} \sim \gD_k } g( \vx^{(k)}, \zeta^{(k)} ) $.
Then we have $f(\vx) = \sE_{\zeta \sim \gD} f(\vx, \zeta) = \frac{1}{N} \sum_{k=1}^N g_k (\vx^{(k)})$,
\[\nabla f(\vx) = \frac{1}{N}
\begin{bmatrix}
\nabla g_1 (\vx^{(1)}) \\
\nabla g_2 (\vx^{(2)}) \\
\vdots \\
\nabla g_N (\vx^{(N)})
\end{bmatrix}
\]
and
\[
\nabla^2 f(\vx) = \frac{1}{N}
\begin{bmatrix}
\nabla^2 g_1 (\vx^{(1)}) & \vzero_d & \cdots & \vzero_d \\
\vzero_d & \nabla^2 g_2 (\vx^{(2)}) & \cdots & \vzero_d \\
\vdots & \vdots & \ddots & \vdots \\
\vzero_d & \vzero_d & \cdots & \nabla^2 g_N (\vx^{(N)})
\end{bmatrix}.
\]


We first focus on Proposition \ref{prop:f(x)}.
Note that the solution to \eqref{eq:dis_opt} must be of the form
\[\vx^\star = \left[ (\vx^{(\star)} )^\top, ( \vx^{(\star)} )^\top, \dots, ( \vx^{(\star)} )^\top   \right]^\top \in \sR^{Nd}.\]

Proposition \ref{prop:f(x)} implies that the solution satisfies $\frac{1}{N} \sum_{k=1}^N \nabla g_k ( \vx^{(\star)} ) = \vzero$.
This equation does not imply that the $\nabla g_k (\vx^{\star})$ are all equal to  zero. In fact, under the heterogeneous setting, where the $g_k$ are different due to the diversity across the clients, we typically have $\nabla f (\vx^{(\star)}) \neq \vzero$.
This is crucial for the validity of Theorem \ref{thm:jump_approx} and Theorem \ref{thm:asy_bias_u}. 
As for the homogeneous setting where the $g_k$ share the same form, $\frac{1}{N} \sum_{k=1}^N \nabla g_k ( \vx^{(\star)} ) = \vzero$ does imply $\nabla g_k (\vx^{(\star)}) = \vzero$ and consequently $\nabla f(\vx^{\star}) = \vzero$. In this case,  Theorem \ref{thm:jump_approx} and \ref{thm:asy_bias_u} do not hold anymore. However, the homogeneous setting is beyond the scope of our paper and is left for future work.
Thus, we assume $\nabla f(\vx^\star) \neq \vzero$ from now on.

Now we turn to the results in Section \ref{sec:converge}.
With $\gP_{\mA^\bot}$ 
% and $\gP_{\mA}$ 
described in \eqref{eq:proj_A_bot_fl},
% and \eqref{eq:proj_A_fl},
we have
\[\vu_n = \left[ (\bar{\vx}_{n} )^\top, ( \bar{\vx}_{n} )^\top, \dots, ( \bar{\vx}_{n} )^\top   \right]^\top,\]
where
$\bar{\vx}_{n} =  \frac{1}{N} \sum_{k=1}^N \vx_{n}^{(k)} $.
As a result, $\sE \norm{ \vu_n - \vx^\star }^2 = N \sE \norm{ \bar{\vx}_n - \vx^{(\star)} }^2$. Then Theorem \ref{thm:converge} guarantees that $\sE \norm{ \bar{\vx}_n - \vx^{(\star)} }^2 = \gO ( n^{- \alpha \min \{ 1 , 2 - 2 \beta \}} ) $, which is what we desire. The revision of Theorem \ref{thm:counter} is deferred to the last part of this subsection.

As for the results in Section \ref{sec:dynamics_approx}, we first take a glance at Theorem \ref{thm:diff_approx}.
Since the expression of $\gP_{\mA^\bot}$ implies we can just focus on the first $d$ dimensions of \eqref{eq:diff_approx}, Theorem \ref{thm:diff_approx} actually characterize the asymptotic behavior of $ \frac{ \bar{\vx}_n - \vx^{(\star)} }{ \sqrt{\eta_{n-1} } } $ when $\beta \in [0, \frac{1}{2}) $.
Then we consider the bias vector mentioned in Theorem \ref{thm:asy_bias_u}.
Direct computation shows
\begin{align*}
    \gP_{\mA^\bot} \nabla^2 f (\vx^\star) \nabla f(\vx^\star)
    & = \frac{1}{N^2}
    \gP_{\mA^\bot}
    \begin{bmatrix}
    \nabla^2 g_1 (\vx^{ (\star) }) \nabla g_1 ( \vx^{ (\star) } ) \\
    \nabla^2 g_2 (\vx^{ (\star) }) \nabla g_2 ( \vx^{ (\star) } ) \\
    \vdots \\
    \nabla^2 g_N (\vx^{ (\star) }) \nabla g_N ( \vx^{ (\star) } ) 
    \end{bmatrix} \\
    & = \frac{1}{N^3}
    \begin{bmatrix}
    \rmI_d \\
    \rmI_d \\
    \vdots \\
    \rmI_d
    \end{bmatrix}
    \sum_{k=1}^N \nabla^2 g_k (\vx^{ (\star) }) \nabla g_k ( \vx^{ (\star) } ).
\end{align*}
Even if $\nabla g_k (\vx^{(\star)}) \neq 0$ for any $k$, the bias vector could still be equal to the zero vector. For example, $\nabla^2 g_k (\vx^{(\star)})$ are all the same and $\sum_{k=1}^N \nabla g_k (\vx^{(\star)}) = \vzero$.
For such a special case, the convergence of $\sE \norm{ \bar{\vx}_n - \vx^{(\star)} }_2^2$ could be faster, since the leading term hindering the convergence vanishes. 


\subsubsection{Revision of the Lower Bound }\label{sec:sp_fedavg_lower}
Finally, we present a revised version of Theorem \ref{thm:counter}.
Recall that the Hessian matrix $\nabla^2 f(\vx)$ is a block diagonal matrix.
Although Theorem \ref{thm:converge} provides a counter example for the general case, it does not specify the form of $\nabla^2 f(\vx)$.
Fortunately, with $\mA$ defined in \eqref{eq:mat_A_fl}, we can find a counter example such that $\nabla^2 f(\vx)$ is a diagonal matrix.
\begin{corollary}
\label{cor:counter}
Consider the problem \eqref{eq:dis_opt}.
If $\eta_n = \eta_0 n^{- \alpha}$ and $p_n = \min\{ p_0 \eta_n, 1 \}$ with $0 < \alpha \le 1$, then there exists a quadratic function $f(\vx)$ such that $ \nabla^2 f(\vx) $ is a diagonal matrix, $\nabla^2 f(\vx) \succeq \rmI_d$ and $\sE \norm{ \vu_n - \vx^\star }^2$ does not converge to $0$. 
\end{corollary}
The proof of Corollary \ref{cor:counter} is deferred to Appendix \ref{sec:append_counter}.

\subsection{Related Work}
In this section, we focus on several works that investigate the asymptotic and dynamical nature of distributed optimization. 
We can trace this line of research back from the classical work \citep{kushner1987asymptotic} by Kushner et al. 
Unlike the prevailing federated learning algorithm (multi-step local computation between adjacent communications), Kushner et al.~\citep{kushner1987asymptotic} consider a random, incomplete decentralized communication within each iteration. And the randomness of these communications are characterized by a sequence of random gossip matrices $\{\rmW_n\}$. In particular, the algorithm has the following form,
\begin{equation}
\begin{aligned}
 \text{Local step:} ~~& \vx_{n+\frac{1}{2},i} = \vx_{n,i} + \epsilon\rmY_{n,i}\\ 
 \text{Gossip step:} ~~& \vx_{n+1,i} = \ssum{j}{1}{N}\omega_{n+1}(i,j)\vx_{n+\frac{1}{2},j}
\end{aligned}
\end{equation}
where $\rmW_n = [\omega_n(i,j)]_{i,j=1}^N$ and $N$ is the number of nodes.

For the algorithm, Kushner et al.~\citep{kushner1987asymptotic} proved that the trajectories of the final iteration converge weakly to the solution of the particular ODE as the step size $\epsilon$ converges to zero, and formally discussed the weak convergence of the rescaled sequences to the solution of a specific linear SDE (i.e. the diffusion approximation result). However, there are several limitations to this work. First of all, the most critical point is that the above theoretical results are discussed in the case of fixed step sizes. As the iteration increases, the variance term of a stochastic approximation begins to dominate the rate of convergence, and the use of a constant step size at this point will make the effect of variance never fall to zero. 
So a fixed step size means a fixed and finite total iteration (depending on the constant step size and the required estimation accuracy). 
This makes all the asymptotic results in 
\citep{kushner1987asymptotic} less practical. 
In addition, the article assumes (without proof) some intermediate results such as tightness and weak convergence at the initial point, making his theoretical results incomplete.

Thereafter, Bianchi et al.~\citep{bianchi2013performance} consider the same random gossip stochastic approximation algorithm. Unlike \citep{kushner1987asymptotic}, Bianchi et al. replace the fixed step size with a decreasing step size and obtain the asymptotic normality of rescaled final iteration and Polyak-Ruppert averaging sequence. 
But note that Bianchi et al.~\citep{bianchi2013performance} assume that all gossip matrices have the same distribution, implying that their asymptotic results hold only if the communication frequency does not decrease as the iteration increases. 
This is equivalent to the case in LPSA where the projection probability is set as a constant. 
In particular, they assume the step size $\gamma_n \sim \frac{1}{n^\alpha}$ satisfies that $\alpha \in (\frac{1}{2},1]$.
In the end, neither of the above two works analyzes the effect of communication frequency on the asymptotic performance of the distributed stochastic approximation algorithm, which is explicitly reflected in our analysis in the form of bias-variance tradeoff.
